Predictive Second Order Sliding Control of Constrained Linear Systems with Application to Automotive Control Systems

This paper presents a new predictive second order sliding controller (PSSC) formulation for setpoint tracking of constrained linear systems. The PSSC scheme is developed by combining the concepts of model predictive control (MPC) and second order discrete sliding mode control. In order to guarantee the feasibility of the PSSC during setpoint changes, a virtual reference variable is added to the PSSC cost function to calculate the closest admissible set point. The states of the system are then driven asymptotically to this admissible setpoint by the control action of the PSSC. The performance of the proposed PSSC is evaluated for an advanced automotive engine case study, where a high fidelity physics-based model of a reactivity controlled compression ignition (RCCI) engine is utilized to serve as the virtual test-bed for the simulations. Considering the hard physical constraints on the RCCI engine states and control inputs, simultaneous tracking of engine load and optimal combustion phasing is a challenging objective to achieve. The simulation results of testing the proposed PSSC on the high fidelity RCCI model show that the developed predictive controller is able to track desired engine load and combustion phasing setpoints, with minimum steady state error, and no overshoot. Moreover, the simulation results confirm the robust tracking performance of the PSSC during transient operations, in the presence of engine cyclic variability.

==> CaseStudies.tex <==
\section{Case Studies} \label{sec:CS}\vspace{-0.15cm}
Here, application of the proposed method in Section~\ref{sec:UncertaintyPrediction} is demonstrated for one linear (DC motor) and one nonlinear (SI engine) case studies. Our proposed algorithm fits the requirements of these automotive control problems well, as they contain complicated plant model dynamics prone to uncertainty in slowly-fluctuating environments, yet require uncertainty mitigation to achieve tracking of desired trajectory behavior.\vspace{-0.15cm}
%
\subsection{Linear Case Study: DC Motor Speed Control} \label{CS_DCMotor} \vspace{-0.10cm}
DC motors are common automotive actuators for control applications that require rotary and transitional motions. For speed regulation of a DC motor, the control input is voltage ($V$) to the motor's armature and the output is rotation speed (${\theta}$) of the shaft. Assuming a constant magnetic field and linear relationship between motor torque and armature current ($\mathcal{I}$), by choosing the rotor speed and current as the state variables, the following discretized linear time-invariant state-space representation can be used to describe the dynamics of the DC motor~\cite{DCMotor_ref}, in which $\alpha_{pq}$ represents the unknown multiplicative term on the plant's parameters: \vspace{-0.25cm}
%
\begin{subequations}
\begin{gather}\label{eq:DC_motor_linear_DSMC_Uncertain}
\theta(k+1)=T\left([-{\alpha}_{11}\frac{k_f}{J}]\theta(k)\right) \\
+T\left(\frac{k_m}{J}{\mathcal{I}}(k)+\frac{1}{J} \Gamma\right) +\theta(k) \nonumber \\
{\mathcal{I}}(k+1)=T\left([-\alpha_{21}\frac{k_b}{L}]\theta(k)+[-\alpha_{22}\frac{R}{L}]{\mathcal{I}}(k)\right)\\
+\frac{T}{L}V(k)+{\mathcal{I}}(k) \nonumber
\end{gather}
\end{subequations}
%
where $J$ is the rotor's moment of inertia, $R$ is the electrical resistance, $L$ is the electric inductance, $\Gamma$ is the generated torque on the rotor, $k_f$ is the mechanical damping, $k_m$ is the motor torque constant, and $k_b$ is the electromotive force constant. The DC motor model constants are listed in %Table~\ref{tab:DC_motor_constants} in %
the Appendix. Three multiplicative ($\alpha_{pq}$) unknown parameters are derived to their nominal values by solving the adaptation law in Eq.~(\ref{eq:D2SMC_14}). A second order DSMC is designed to regulate the DC motor rotational speed with respect to the desired speed profile ($\theta_d$). The first sliding surface is defined as the error in tracking the desired speed profile ($s_{1}=\theta-\theta_d$). Since there is no direct control input on DC motor rotational speed, $\mathcal{I}_d$ is defined as the synthetic control input for controlling the shaft speed. $\mathcal{I}_d$ is used to define the second sliding surface ($s_{2}=\mathcal{I}-\mathcal{I}_d$) in which the control input is voltage. The final synthetic ($\mathcal{I}_d$) and physical ($V$) control inputs are calculated as follows: \vspace{-0.25cm}
%
\begin{subequations} \label{eq:DC_motor_adaptiveDSMC_modified}
\begin{gather}
{\mathcal{I}}_d(k)=\frac{J}{k_m}\left(\frac{1}{T}\left[-\beta_1(\theta(k)-\theta_d(k))+\theta_d(k+1)\right.\right.\\
\left.\left.-\theta(k)\right]+[\hat{\alpha}_{11}\frac{k_f}{J}\theta(k)]-\frac{1}{J}\Gamma\right) \nonumber \\
%
V(k)=L\left(\frac{1}{T_s}\left[-\beta_2({\mathcal{I}}(k)-{\mathcal{I}}_d(k))+{\mathcal{I}}_d(k+1)
\right.\right.\\
\left.\left.-{\mathcal{I}}(k)\right] 
+[\hat{\alpha}_{21}\frac{k_b}{L}]\theta(k)+\hat{\alpha}_{22}\frac{R}{L}{\mathcal{I}}(k)\right) \nonumber
\end{gather} %\vspace{-1cm}
\end{subequations}
%%
Simulations are done in MATLAB Simulink$^{\textregistered}$~which allows for testing the controller in a model-in-the-loop (MIL) platform for different sampling rates. In the absence of model uncertainties ($\alpha_{pq}=1$), Fig.~\ref{fig:DC_2DSMC_SamplingComparison} shows the comparison between the first~\cite{Pan_Discrete} and second order DSMCs for different sampling rates. Although at lower sampling rates (e.g., $200~ms$) both controllers show similar performances, by increasing the sampling rate to $800~ms$, the higher robustness characteristics of the second order DSMC in comparison with the first order controller are revealed. The comparison results show that the second order DSMC is improving the tracking errors by 69\% on average for different sampling rates, compared to the first order DSMC.\vspace{-0.35cm}
%%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{DC_2DSMC_SamplingComparison.eps} \vspace{-0.85cm}
\caption{\label{fig:DC_2DSMC_SamplingComparison}Comparison between the first and second order DSMCs in tracking the desired speed trajectory of the DC motor for different sampling rates. (a) First order DSMC, (b) Second order DSMC. Values inside the parentheses show the resulting improvement ($\downarrow$) from the second order DSMC compared to the first order DSMC.} \vspace{-0.55cm}
\end{center}
\end{figure}
%

The convergence results of the unknown parameters are shown in Fig.~\ref{fig:DC_2DSMC_ParamConv}. This is done by simultaneously solving Eq.~(\ref{eq:D2SMC_14}) and Eq.~(\ref{eq:DC_motor_adaptiveDSMC_modified}). The performance of the first~\cite{Amini_DSCC2016}, and second order adaptive DSMCs are shown in Fig.~\ref{fig:DC_2DSMC_SpeedTracking} for tracking the desired speed profile under 200 $ms$ of sampling time, and up 50\% uncertainty on the plant's parameters. As can be observed, the second order DSMC is able to significantly improve the tracking performance by 60\% compared to the first order adaptive DSMC.\vspace{-0.45cm}
%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{DC_2DSMC_ParamConv.eps} \vspace{-0.85cm}
\caption{\label{fig:DC_2DSMC_ParamConv}Convergence results of the unknown multiplicative ($\alpha$) terms in the DC motor model (sampling time=200 ms).} \vspace{-0.75cm}
\end{center}
\end{figure}
%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{DC_2DSMC_SpeedTracking.eps} \vspace{-0.85cm}
\caption{\label{fig:DC_2DSMC_SpeedTracking}DC motor speed control using the first and second order \textit{adaptive} DSMCs (sampling time=200 ms).} \vspace{-1cm}
\end{center}
\end{figure}
%----------------------------------------------------------------
\subsection{Nonlinear Case Study: Automotive Engine Control}\label{subsec:Engine_Control}\vspace{-0.10cm}
%
%The effectiveness of adaptive control strategy for engine and powertrain controls has been demonstrated in the literature~\cite{JingSun_1,JingSun_2}. 
In this section, the performance of the proposed adaptive second order DSMC is studied for a physics-based spark ignition (SI) combustion engine model~\cite{Shaw} during cold start. The engine model~\cite{Shaw} is parameterized for a 2.4-liter, 4-cylinder, DOHC 16-valve Toyota 2AZ-FE engine. The engine rated power is 117kW $@$ 5600~RPM, and it has a rated torque of 220 Nm $@$ 4000~RPM. The experimental validation of different components of the engine model is available in~\cite{Sanketi}. The nonlinear model has four states including the exhaust gas temperature~($T_{exh}$), fuel mass flow rate into the cylinders (${\dot{m}_f}$), the engine speed~(${\omega_e}$), and the mass of air inside the intake manifold ($m_{a}$). The control problem is defined to steer $T_{exh}$, ${\omega_e}$, and air-fuel ratio ($AFR$) to their pre-defined desired values. A set of four SISO DSMCs is designed to achieve this objective. Four states of the model and corresponding dynamics and controllers will be discussed in the following sections. Details of the functions and constants in the engine model are found in the Appendix and~\cite{Sanketi}. 
%

%\vspace{0.15cm}%-----------------------
$\bullet {\textbf{~~Exhaust~Gas~Temperature~Controller:}}$~Discretized model for exhaust gas temperature ($T_{exh}$) is:
%
\vspace{-0.2cm}
\begin{gather}
\label{eq:Engine_discretized_1}
T_{exh}(k+1)=(1-\frac{T}{\tau_e})T_{exh}(k)\\
+\frac{T}{\tau_e}(7.5\Delta(k)+600)AFI(k)  \nonumber
\end{gather}
%
where $\Delta(k)$ is the control input. The sliding surface for $T_{exh}$ controller is defined to be the error in tracking the desired exhaust gas temperature ($s_{1}=T_{exh}-{T_{exh,d}}$). The dynamics of the exhaust gas temperature ($f_{{T_{exh}}}$) with multiplicative unknown term ($\alpha_{T_{exh}}$) is: \vspace{-0.20cm}
%
\begin{gather}
\label{eq:Engine_discretized_Texh}
f_{{T_{exh}}}=\alpha_{T_{exh}}\Big(\frac{1}{\tau_e}[600AFI-T_{exh}]\Big)
\end{gather}
%
The exhaust gas time constant ($\tau_{e}$) has a significant role in the exhaust gas temperature dynamics (Eq.~(\ref{eq:Engine_discretized_Texh})). This means that any error in estimating the time constant ($\tau_{e}$) directly affects the dynamics and causes deviation from the nominal model. Multiplicative uncertainty term ($\alpha_{T_{exh}}$) is assumed to represent any error in estimating $\tau_{e}$. The error in the modeled $T_{exh}$ dynamics is removed by using the following adaptation law with respect to Eq.~(\ref{eq:D2SMC_14}): \vspace{-0.15cm}
%
\begin{gather}
\label{eq:adaptive_Texh}
\hat{\alpha}_{T_{exh}}(k+1)=\hat{\alpha}_{T_{exh}}(k)+\frac{T(s_1(k))}{\tau_e \rho_{\alpha_1}}(600AFI-T_{exh}(k))
\end{gather}
%
By incorporating Eq.~(\ref{eq:Engine_discretized_1}) and $\hat{\alpha}_{T_{exh}}$ from Eq.~(\ref{eq:adaptive_Texh}) into Eq.~(\ref{eq:D2SMC_6}), the second order adaptive DSMC for exhaust gas temperature becomes: \vspace{-0.25cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_1}
\Delta(k)=\frac{\tau_e}{7.5\,.\,AFI\,.\,T}[-\hat{\alpha}_{T_{exh}}(k)\frac{T}{\tau_e}(600\,.\,AFI\\
-T_{exh}(k))-(\beta_1+1)s_1(k)+T_{exh,d}(k+1)-T_{exh,d}(k)] \nonumber
\end{gather} \vspace{-0.75cm}
%

%\vspace{0.15cm}%----------------------------------------------------
$\bullet { \textbf{~~Fuel~Flow~Rate~Controller:}}$~The discretized difference equation for the fuel flow rate is: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_2}
\dot{m}_f(k+1)=\dot{m}_f(k)+\frac{T}{\tau_f}[\dot{m}_{fc}(k)-\dot{m}_f(k)]
\end{gather}
%
The fuel flow dynamic ($f_{\dot{m}_f}$) with multiplicative uncertainty term ($\alpha_{\dot{m}_f}$) is as follows: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_mdotf}
f_{\dot{m}_f}=-\alpha_{\dot{m}_f}\Big(\frac{1}{\tau_f}\dot{m}_f(k)\Big) 
\end{gather}
%
The sliding variable for the fuel flow controller is defined to be the error in tracking the desired fuel mass flow ($s_{2}={\dot{m}_{f}}-{\dot{m}_{f,d}}$). In a similar manner to $T_{exh}$ dynamics, the fuel evaporation time constant $\tau_{f}$ dictates the dynamics of the fuel flow into the cylinder. Consequently, any error in estimating $\tau_{f}$ leads to a considerable deviation from the nominal model. $\alpha_{\dot{m}_f}$ is introduced to the fuel flow dynamics to represent the uncertainty in estimating $\tau_{f}$. The adaptation law for $\alpha_{\dot{m}_f}$ becomes:  
\vspace{-0.4cm}
%
\begin{gather}
\label{eq:adaptive_mdotf}
\hat{\alpha}_{\dot{m}_f}(k+1)=\hat{\alpha}_{\dot{m}_f}(k)-\frac{T(s_2(k))}{\tau_f \rho_{\alpha_2}}\dot{m}_f(k)
\end{gather}
%
where, $\dot{m}_{f,d}$ is calculated according to desired AFR. The adaptive control law for $\dot{m}_{fc}$ is: \vspace{-0.15cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_2}
\dot{m}_{fc}(k)=\frac{\tau_f}{T}[\hat{\alpha}_{\dot{m}_f}(k)\frac{T}{\tau_f}\dot{m}_f(k) \\-(\beta_2+1)s_2(k)+\dot{m}_{f,d}(k+1)-\dot{m}_{f,d}(k)] \nonumber
\end{gather} \vspace{-0.75cm}
%

%\vspace{0.15cm}%-----------------------
$\bullet { \textbf{~~Engine~Speed~Controller:}}$~The rotational dynamics of the engine is described by using the following difference equation:\vspace{-0.4cm}
%
\begin{gather}
\label{eq:Engine_discretized_3}
\omega_e(k+1)=\omega_e(k)+\frac{T}{J}T_E(k) 
\end{gather}
%
where $T_E(k)$ is the engine torque and is found by $30000~m_a(k)-(0.4~\omega_e(k)+100)$. There is no direct control input for modulating the engine speed, therefore $m_a$ is considered as the synthetic control input. The calculated $m_a$ from engine speed controller will be used as the desired trajectory in intake air mass flow rate controller. $f_{\omega_e}$ of the engine with multiplicative uncertainty ($\alpha_{\omega_e}$) is as follows: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_we}
f_{\omega_e}=-\alpha_{\omega_e}\Big(\frac{1}{J}T_{loss}\Big)
\end{gather} 
%
where $T_{loss}=0.4\omega_e+100$. $T_{loss}$ represents the torque losses on the crankshaft. Thus, the multiplicative uncertainty $\alpha_{\omega_e}$ compensates for any error in estimated torque loss. The sliding variable for the engine speed controller is defined to be $s_3=\omega_e-{\omega_{e,d}}$. $\alpha_{\omega_e}$ is driven to ``1'' using the following adaptation law: \vspace{-0.3cm}
%
\begin{gather}
\label{eq:adaptive_we}
\hat{\alpha}_{\omega_e}(k+1)=\hat{\alpha}_{\omega_e}(k)-\frac{T(s_3(k))}{J.\rho_{\alpha_3}}(0.4\omega_e(k)+100)
\end{gather}
%
Finally, the desired synthetic control input ($m_{a,d}$) is:\vspace{-0.3cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_3}
m_{a,d}(k)=\frac{J}{30,000\,T}[\hat{\alpha}_{\omega_e}(k)\frac{T}{J}(100+0.4\omega_e(k))\\\nonumber-(\beta_3+1)s_3(k)  
+\omega_{e,d}(k+1)-\omega_{e,d}(k)]
%\end{split}
\end{gather} %\vspace{-1cm}
%

%\vspace{0.15cm} %------------------------------------------
$\bullet { \textbf{~~Air~Mass~Flow~Controller:}}$
%
The following state difference equation describes the air mass flow behaviour in discrete time: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_3}
m_a(k+1)=m_a(k)+T[\dot{m}_{ai}(k)-\dot{m}_{ao}(k)]
\end{gather}
%
The calculated $m_{a,d}$ from Eq.~(\ref{eq:Engine_DSMC_Final_3}) is used as the desired trajectory to obtain $\dot{m}_{ai}$ as the control input of $m_a$ controller. The last sliding surface for the air mass flow controller is defined to be $s_4=m_a-{m_{a,d}}$. The intake air manifold mass dynamic with the unknown term ($\alpha_{m_a}$) is: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_ma}
f_{m_a}=-\alpha_{m_a}\dot{m}_{ao}(k)
\end{gather}  \vspace{-0.35cm}
%
where, air mass flow into the cylinder is determined by~\cite{Shaw}: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_ma2}
\dot{m}_{ao}=k_1\eta_{vol}m_a\omega_e 
%\label{eq:Engine_discretized_ma3}
%\eta_{vol}=m_a^2(k_2{\omega_e^2}+k_3\omega_e+k_4)+m_a(k_5{\omega_e^2}+k_6\omega_e+k_7) \\ \nonumber 
%+k_8{\omega_e^2}+k_9{\omega_e}+k_{10}% \nonumber
\end{gather}
%
$\eta_{vol}$ is the volumetric efficiency. As can be seen from Eq.~(\ref{eq:Engine_discretized_ma}) and~(\ref{eq:Engine_discretized_ma2}), the multiplicative uncertainty term in the intake air manifold dynamics ($\alpha_{m_a}$) represents the uncertainty in $\dot{m}_{ao}$ that is extracted from $\eta_{vol}$ map. $\alpha_{m_a}$ is updated using the following adaptation law:  \vspace{-0.2cm}
%
\begin{gather}
\label{eq:adaptive_ma}
\hat{\alpha}_{m_a}(k+1)=\hat{\alpha}_{m_a}(k)-\frac{T(s_4(k))}{\rho_{\beta_4}}\dot{m}_{ao}
\end{gather}
%
Finally, the controller input is:  \vspace{-0.2cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_4}
\dot{m}_{ai}(k)=\frac{1}{T}[\hat{\alpha}_{m_a}(k)\dot{m}_{ao}(k)T-(\beta_4+1)s_4(k)\\
+m_{a,d}(k+1)-m_{a,d}(k)] \nonumber
\end{gather}
%
In the absence of model uncertainties ($\alpha_{T_{exh}}=\alpha_{\dot{m}_f}=\alpha_{\omega_e}=\alpha_{{m}_a}=1$), Fig.~\ref{fig:Engine_2DSMC_SamplingComparison_10ms} and~\ref{fig:Engine_2DSMC_SamplingComparison_40ms} show the results of tracking the desired $AFR$, $T_{exh}$, and engine speed trajectories, using the first and second order DSMCs for sampling times of $10~ms$ and $40~ms$, respectively. The mean tracking errors for both controllers are listed in Table~\ref{table:tracking_Results}. It can be observed from Fig.~~\ref{fig:Engine_2DSMC_SamplingComparison_10ms} and Table~\ref{table:tracking_Results} when the signals at the controller I/O are sampled every $10~ms$, both first and second order DSMCs illustrate acceptable tracking performances, while the second order controller is 50\% more robust on average in terms of the tracking errors. Upon increasing the sampling rate from $10~ms$ to $40~ms$, the first order DSMC performance degrades significantly. On the other side, despite the increase in the sampling time, the second order DSMC still presents smooth and accurate tracking results. By comparing the first and second order DSMC results at $T=40~ms$, it can be concluded that the proposed second order DSMC outperforms the first order controller by up to 85\% in terms of the mean tracking errors.  %\vspace{-0.35cm}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_SamplingComparison_10ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_SamplingComparison_10ms}Engine tracking results by the first and second order DSMCs with $T=10~ms$.} \vspace{-0.55cm}
\end{center}
\end{figure}
%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_SamplingComparison_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_SamplingComparison_40ms}Engine tracking results by the first and second order DSMCs with $T=40~ms$.} \vspace{-0.40cm}
\end{center}
\end{figure} 
%
\begin{table} [htbp!]
\small
\begin{center}
\caption{Mean ($\bar{e}$) of Tracking Errors. Values Inside the Parentheses Show the Resulting Improvement from the Second Order DSMC Compared to the First Order DSMC.} \linespread{1.15}
\label{table:tracking_Results}\vspace{-0.15cm}
\begin{tabular}{lccccc}
        \hline\hline
\multicolumn{1}{c}{} & \multicolumn{2}{c}{$\bar{e}~(T=10~ms)$}                                                        &  & \multicolumn{2}{c}{$\bar{e}~(T=40~ms)$} \\
\cline{2-3} \cline{5-6}
\textbf{}& {$1^{st}$-Order} & {$2^{nd}$-Order} &  & {$1^{st}$-Order}  & {$2^{nd}$-Order} \\
\textbf{}& {DSMC} & {DSMC} &  & {DSMC}  & {DSMC} \\
\textbf{}   & {\textcolor{blue}{Reference}}& \textbf{}  &  & {\textcolor{blue}{Reference}} & \textbf{}  \\ \hline
AFR& 0.028  &  0.010   &    &  0.126   &  0.019       \\ \vspace{0.05cm}
[-]        &        & \textcolor{blue}{(-64\%)} &  &  & \textcolor{blue}{(-84.9\%)} \\ \hline \vspace{0.05cm} 
$T_{exh}$ & 0.2  & 0.1  &  & 1.8 & 0.2 \\ \vspace{0.05cm}
[$^o$C]                 &      & \textcolor{blue}{(-50\%)} &  &  & \textcolor{blue}{(-88.9\%)}\\ \hline \vspace{0.05cm} 
$N$  & 0.1  &   0.06   &  &   1.9    & 0.3\\ \vspace{0.05cm}
 [RPM]                &      & \textcolor{blue}{(-40\%)} &  &  & \textcolor{blue}{(-84.2\%)} \\ 
\hline\hline 
\end{tabular} \vspace{-0.5cm}
\end{center}
\end{table}
\linespread{1} 

The effect of the unknown multiplicative terms (up to 25\%) on the engine plant's dynamics ($f$) is shown in Fig.~\ref{fig:Engine_2DSMC_DynamicImpact_40ms}. The uncertainty terms in the model introduce a permanent error in the estimated dynamics compared to the nominal model. If these errors are not removed in the early seconds of the controller operation, the tracking performance will be affected adversely. Upon activation of the adaptation mechanism, as it can be observed from Fig.~\ref{fig:Engine_2DSMC_DynamicImpact_40ms}, the model with error is steered towards the nominal model in less than 2 $sec$. Consequently, the errors in the model are removed. Fig.~\ref{fig:Engine_2DSMC_ParamConv_40ms} shows the results of unknown multiplicative uncertainty term ($\hat{\alpha}$) estimation against the actual (nominal) values ($\alpha$). %\vspace{-0.4cm}

%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_DynamicImpact_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_DynamicImpact_40ms}The effect of the model uncertainty terms on the engine dynamics when using the second order DSMC and how the adaptation mechanism drives the model with error to its nominal value: (a) $T_{exh}$, (b) $\dot{m}_f$, (c) $\omega_e$, and (d) $m_a$ ($T=40~ms$).} \vspace{-0.55cm}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_ParamConv_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_ParamConv_40ms}Estimation of unknown multiplicative parameters in adaptive DSMC ($T=40~ms$).} \vspace{-0.55cm}
\end{center}
\end{figure}

Fig.~\ref{fig:Engine_2DSMC_AdaptiveTracking_40ms} shows the comparison between the tracking performances of the non-adaptive and adaptive second order DSMCs. As expected, the non-adaptive DMSC fails to track the desired trajectories, which explains the importance of handling the model uncertainties in the body of the DSMC. On the other hand, once the adaptation algorithm is enabled and the convergence period of the unknown parameters is over, the adaptive DSMC tracks all the desired trajectories smoothly with the minimum error under $40~ms$ sampling time.% ($N$ is the engine speed in terms of $RPM$). 
\vspace{-0.4cm}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_AdaptiveTracking_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_AdaptiveTracking_40ms}Comparison between adaptive and non-adaptive second order DSMCs for the engine model with uncertainties: (a) $AFR$, (b) $T_{exh}$, and (c) $N$~($T=40~ms$).} \vspace{-0.75cm}
\end{center}
\end{figure}



==> CaseStudies2.tex <==
\section{Case Study: Automotive Engine Control} 
\label{sec:CS}\vspace{-0.15cm}
Here, application of the proposed method in Section~\ref{sec:UncertaintyPrediction} is demonstrated for a physics-based spark ignition (SI) combustion engine model~\cite{Shaw} during cold start. Our proposed algorithm fits the requirements of this automotive control problem well, as it contains complicated plant model dynamics prone to uncertainty in slowly-fluctuating environments, yet require uncertainty mitigation to achieve tracking of desired trajectory behavior.%\vspace{-0.15cm}

%----------------------------------------------------------------
%\subsection{Nonlinear c}\label{subsec:Engine_Control}\vspace{-0.10cm}
%
%The effectiveness of adaptive control strategy for engine and powertrain controls has been demonstrated in the literature~\cite{JingSun_1,JingSun_2}. 
The engine model~\cite{Shaw} is parameterized for a 2.4-liter, 4-cylinder, DOHC 16-valve Toyota 2AZ-FE engine. The engine rated power is 117kW $@$ 5600~RPM, and it has a rated torque of 220 Nm $@$ 4000~RPM. The experimental validation of different components of the engine model is available in~\cite{Sanketi}. The nonlinear model has four states including the exhaust gas temperature~($T_{exh}$), fuel mass flow rate into the cylinders (${\dot{m}_f}$), the engine speed~(${\omega_e}$), and the mass of air inside the intake manifold ($m_{a}$). The control problem is defined to steer $T_{exh}$, ${\omega_e}$, and air-fuel ratio ($AFR$) to their pre-defined desired values. A set of four SISO DSMCs is designed to achieve this objective. Four states of the model and corresponding dynamics and controllers will be discussed in the following sections. Details of the functions and constants in the engine model are found in the Appendix and~\cite{Sanketi}. 
%

%\vspace{-0.01cm}%-----------------------
$\bullet {\textbf{~~Exhaust~Gas~Temperature~Controller:}}$~Discretized model for exhaust gas temperature ($T_{exh}$) is:
%
\vspace{-0.2cm}
\begin{gather}
\label{eq:Engine_discretized_1}
T_{exh}(k+1)=(1-\frac{T}{\tau_e})T_{exh}(k)\\
+\frac{T}{\tau_e}(7.5\Delta(k)+600)AFI(k)  \nonumber
\end{gather}
%
where $\Delta(k)$ is the control input. The sliding surface for $T_{exh}$ controller is defined to be the error in tracking the desired exhaust gas temperature ($s_{1}=T_{exh}-{T_{exh,d}}$). The dynamics of the exhaust gas temperature ($f_{{T_{exh}}}$) with multiplicative unknown term ($\alpha_{T_{exh}}$) is: \vspace{-0.20cm}
%
\begin{gather}
\label{eq:Engine_discretized_Texh}
f_{{T_{exh}}}=\alpha_{T_{exh}}\Big(\frac{1}{\tau_e}[600AFI-T_{exh}]\Big)
\end{gather}
%
The exhaust gas time constant ($\tau_{e}$) has a significant role in the exhaust gas temperature dynamics (Eq.~(\ref{eq:Engine_discretized_Texh})). This means that any error in estimating the time constant ($\tau_{e}$) directly affects the dynamics and causes deviation from the nominal model. Multiplicative uncertainty term ($\alpha_{T_{exh}}$) is assumed to represent any error in estimating $\tau_{e}$. The error in the modeled $T_{exh}$ dynamics is removed by using the following adaptation law with respect to Eq.~(\ref{eq:D2SMC_14}): \vspace{-0.15cm}
%
\begin{gather}
\label{eq:adaptive_Texh}
\hat{\alpha}_{T_{exh}}(k+1)=\hat{\alpha}_{T_{exh}}(k)+\frac{T(s_1(k))}{\tau_e \rho_{\alpha_1}}(600AFI-T_{exh}(k))
\end{gather}
%
By incorporating Eq.~(\ref{eq:Engine_discretized_1}) and $\hat{\alpha}_{T_{exh}}$ from Eq.~(\ref{eq:adaptive_Texh}) into Eq.~(\ref{eq:D2SMC_6}), the second order adaptive DSMC for exhaust gas temperature becomes: \vspace{-0.25cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_1}
\Delta(k)=\frac{\tau_e}{7.5\,.\,AFI\,.\,T}[-\hat{\alpha}_{T_{exh}}(k)\frac{T}{\tau_e}(600\,.\,AFI\\
-T_{exh}(k))-(\beta_1+1)s_1(k)+T_{exh,d}(k+1)-T_{exh,d}(k)] \nonumber
\end{gather} \vspace{-0.75cm}
%

%\vspace{0.15cm}%----------------------------------------------------
$\bullet { \textbf{~~Fuel~Flow~Rate~Controller:}}$~The discretized difference equation for the fuel flow rate is: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_2}
\dot{m}_f(k+1)=\dot{m}_f(k)+\frac{T}{\tau_f}[\dot{m}_{fc}(k)-\dot{m}_f(k)]
\end{gather}
%
The fuel flow dynamic ($f_{\dot{m}_f}$) with multiplicative uncertainty term ($\alpha_{\dot{m}_f}$) is as follows: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_mdotf}
f_{\dot{m}_f}=-\alpha_{\dot{m}_f}\Big(\frac{1}{\tau_f}\dot{m}_f(k)\Big) 
\end{gather}
%
The sliding variable for the fuel flow controller is defined to be the error in tracking the desired fuel mass flow ($s_{2}={\dot{m}_{f}}-{\dot{m}_{f,d}}$). In a similar manner to $T_{exh}$ dynamics, the fuel evaporation time constant $\tau_{f}$ dictates the dynamics of the fuel flow into the cylinder. Consequently, any error in estimating $\tau_{f}$ leads to a considerable deviation from the nominal model. $\alpha_{\dot{m}_f}$ is introduced to the fuel flow dynamics to represent the uncertainty in estimating $\tau_{f}$. The adaptation law for $\alpha_{\dot{m}_f}$ is:  
\vspace{-0.4cm}
%
\begin{gather}
\label{eq:adaptive_mdotf}
\hat{\alpha}_{\dot{m}_f}(k+1)=\hat{\alpha}_{\dot{m}_f}(k)-\frac{T(s_2(k))}{\tau_f \rho_{\alpha_2}}\dot{m}_f(k)
\end{gather}
%
where, $\dot{m}_{f,d}$ in $s_2$ is calculated according to desired AFR. The adaptive control law for $\dot{m}_{fc}$ is: \vspace{-0.15cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_2}
\dot{m}_{fc}(k)=\frac{\tau_f}{T}[\hat{\alpha}_{\dot{m}_f}(k)\frac{T}{\tau_f}\dot{m}_f(k) \\-(\beta_2+1)s_2(k)+\dot{m}_{f,d}(k+1)-\dot{m}_{f,d}(k)] \nonumber
\end{gather} \vspace{-0.5cm}
%

%\vspace{0.15cm}%-----------------------
$\bullet { \textbf{~~Engine~Speed~Controller:}}$~The rotational dynamics of the engine is described by using the following equation:\vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_3}
\omega_e(k+1)=\omega_e(k)+\frac{T}{J}T_E(k) 
\end{gather}
%
where $T_E(k)$ is the engine torque and is found by $30000~m_a(k)-(0.4~\omega_e(k)+100)$. There is no direct control input for modulating the engine speed, therefore $m_a$ is considered as the synthetic control input. The calculated $m_a$ from engine speed controller will be used as the desired trajectory in intake air mass flow rate controller. $f_{\omega_e}$ of the engine with multiplicative uncertainty ($\alpha_{\omega_e}$) is as follows: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_we}
f_{\omega_e}=-\alpha_{\omega_e}\Big(\frac{1}{J}T_{loss}\Big)
\end{gather} 
%
where $T_{loss}=0.4\omega_e+100$. $T_{loss}$ represents the torque losses on the crankshaft. Thus, the multiplicative uncertainty $\alpha_{\omega_e}$ compensates for any error in estimated torque loss. The sliding variable for the engine speed controller is defined to be $s_3=\omega_e-{\omega_{e,d}}$. $\alpha_{\omega_e}$ is driven to ``1'' using the following adaptation law: \vspace{-0.3cm}
%
\begin{gather}
\label{eq:adaptive_we}
\hat{\alpha}_{\omega_e}(k+1)=\hat{\alpha}_{\omega_e}(k)-\frac{T(s_3(k))}{J.\rho_{\alpha_3}}(0.4\omega_e(k)+100)
\end{gather}
%
Finally, the desired synthetic control input ($m_{a,d}$) is:\vspace{-0.3cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_3}
m_{a,d}(k)=\frac{J}{30,000\,T}[\hat{\alpha}_{\omega_e}(k)\frac{T}{J}(100+0.4\omega_e(k))\\\nonumber-(\beta_3+1)s_3(k)  
+\omega_{e,d}(k+1)-\omega_{e,d}(k)]
%\end{split}
\end{gather} %\vspace{-1cm}
%

%\vspace{0.15cm} %------------------------------------------
$\bullet { \textbf{~~Air~Mass~Flow~Controller:}}$
%
The following state difference equation describes the air mass flow behaviour: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_3}
m_a(k+1)=m_a(k)+T[\dot{m}_{ai}(k)-\dot{m}_{ao}(k)]
\end{gather}
%
The calculated $m_{a,d}$ from Eq.~(\ref{eq:Engine_DSMC_Final_3}) is used as the desired trajectory to obtain $\dot{m}_{ai}$ as the control input of $m_a$ controller. The last sliding surface for the air mass flow controller is defined to be $s_4=m_a-{m_{a,d}}$. The intake air manifold mass dynamic with the unknown term ($\alpha_{m_a}$) is: \vspace{-0.25cm}
%
\begin{gather}
\label{eq:Engine_discretized_ma}
f_{m_a}=-\alpha_{m_a}\dot{m}_{ao}(k)
\end{gather}  \vspace{-0.35cm}
%
where, air mass flow into the cylinder is determined by~\cite{Shaw}: \vspace{-0.2cm}
%
\begin{gather}
\label{eq:Engine_discretized_ma2}
\dot{m}_{ao}=k_1\eta_{vol}m_a\omega_e 
%\label{eq:Engine_discretized_ma3}
%\eta_{vol}=m_a^2(k_2{\omega_e^2}+k_3\omega_e+k_4)+m_a(k_5{\omega_e^2}+k_6\omega_e+k_7) \\ \nonumber 
%+k_8{\omega_e^2}+k_9{\omega_e}+k_{10}% \nonumber
\end{gather}
%
$\eta_{vol}$ is the volumetric efficiency. As can be seen from Eq.~(\ref{eq:Engine_discretized_ma}) and~(\ref{eq:Engine_discretized_ma2}), the multiplicative uncertainty term in the intake air manifold dynamics ($\alpha_{m_a}$) represents the uncertainty in $\dot{m}_{ao}$ that is extracted from $\eta_{vol}$ map. $\alpha_{m_a}$ is updated using the following adaptation law:  \vspace{-0.2cm}
%
\begin{gather}
\label{eq:adaptive_ma}
\hat{\alpha}_{m_a}(k+1)=\hat{\alpha}_{m_a}(k)-\frac{T(s_4(k))}{\rho_{\beta_4}}\dot{m}_{ao}
\end{gather}
%
Finally, the controller input is:  \vspace{-0.2cm}
%
\begin{gather}\label{eq:Engine_DSMC_Final_4}
\dot{m}_{ai}(k)=\frac{1}{T}[\hat{\alpha}_{m_a}(k)\dot{m}_{ao}(k)T-(\beta_4+1)s_4(k)\\
+m_{a,d}(k+1)-m_{a,d}(k)] \nonumber
\end{gather}
%
In the absence of model uncertainties ($\alpha_{T_{exh}}=\alpha_{\dot{m}_f}=\alpha_{\omega_e}=\alpha_{{m}_a}=1$), Figures~\ref{fig:Engine_2DSMC_SamplingComparison_10ms} and~\ref{fig:Engine_2DSMC_SamplingComparison_40ms} show the results of tracking the desired $AFR$, $T_{exh}$, and engine speed trajectories, using the first and second order DSMCs for sampling times of $10~ms$ and $40~ms$, respectively. The mean tracking errors for both controllers are listed in Table~\ref{table:tracking_Results}. It can be observed from Fig.~~\ref{fig:Engine_2DSMC_SamplingComparison_10ms} and Table~\ref{table:tracking_Results} when the signals at the controller I/O are sampled every $10~ms$, both first and second order DSMCs illustrate acceptable tracking performances, while the second order controller is 50\% more robust on average in terms of the tracking errors. As long as the Shannon's sampling theorem criteria, which states that the sampling frequency must be at least twice the maximum frequency of the measured analog signal, is satisfied, increasing the sampling time helps to reduce the computation cost. Upon increasing the sampling rate from $10~ms$ to $40~ms$, the first order DSMC performance degrades significantly. On the other side, despite the increase in the sampling time, the second order DSMC still presents smooth and accurate tracking results. By comparing the first and second order DSMC results at $T=40~ms$, it can be concluded that the proposed second order DSMC outperforms the first order controller by up to 85\% in terms of the mean tracking errors. \vspace{-0.5cm}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_SamplingComparison_10ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_SamplingComparison_10ms}Engine tracking results by the first and second order DSMCs with $T=10~ms$.} \vspace{-0.8cm}
\end{center}
\end{figure}
%
%
\begin{table} [htbp!]
\small
\begin{center}
\caption{Mean ($\bar{e}$) of Tracking Errors. Values Inside the Parentheses Show the Resulting Improvement from the Second Order DSMC Compared to the First Order DSMC.} \linespread{1.15}
\label{table:tracking_Results}\vspace{-0.15cm}
\begin{tabular}{lccccc}
        \hline\hline
\multicolumn{1}{c}{} & \multicolumn{2}{c}{$\bar{e}~(T=10~ms)$}                                                        &  & \multicolumn{2}{c}{$\bar{e}~(T=40~ms)$} \\
\cline{2-3} \cline{5-6}
\textbf{}& {$1^{st}$-Order} & {$2^{nd}$-Order} &  & {$1^{st}$-Order}  & {$2^{nd}$-Order} \\
\textbf{}& {DSMC} & {DSMC} &  & {DSMC}  & {DSMC} \\
\textbf{}   & {\textcolor{blue}{Reference}}& \textbf{}  &  & {\textcolor{blue}{Reference}} & \textbf{}  \\ \hline
AFR& 0.028  &  0.010   &    &  0.126   &  0.019       \\ \vspace{0.05cm}
[-]        &        & \textcolor{blue}{(-64\%)} &  &  & \textcolor{blue}{(-84.9\%)} \\ \hline \vspace{0.05cm} 
$T_{exh}$ & 0.2  & 0.1  &  & 1.8 & 0.2 \\ \vspace{0.05cm}
[$^o$C]                 &      & \textcolor{blue}{(-50\%)} &  &  & \textcolor{blue}{(-88.9\%)}\\ \hline \vspace{0.05cm} 
$N$  & 0.1  &   0.06   &  &   1.9    & 0.3\\ \vspace{0.05cm}
 [RPM]                &      & \textcolor{blue}{(-40\%)} &  &  & \textcolor{blue}{(-84.2\%)} \\ 
\hline\hline 
\end{tabular} \vspace{-0.5cm}
\end{center}
\end{table}
\linespread{1} 
%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_SamplingComparison_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_SamplingComparison_40ms}Engine tracking results by the first and second order DSMCs with $T=40~ms$.} \vspace{-0.8cm}
\end{center}
\end{figure} 
%

The effect of the unknown multiplicative terms (up to 25\%) on the engine plant's dynamics ($f$) is shown in Fig.~\ref{fig:Engine_2DSMC_DynamicImpact_40ms}. The uncertainty terms in the model introduce a permanent error in the estimated dynamics compared to the nominal model. If these errors are not removed in the early seconds of the controller operation, the tracking performance will be affected adversely. Upon activation of the adaptation mechanism, as it can be observed from Fig.~\ref{fig:Engine_2DSMC_DynamicImpact_40ms}, the model with error is steered towards the nominal model in less than 2 $sec$. Consequently, the errors in the model are removed. Fig.~\ref{fig:Engine_2DSMC_ParamConv_40ms} shows the results of unknown multiplicative uncertainty term ($\hat{\alpha}$) estimation against the actual (nominal) values ($\alpha$). \vspace{-0.35cm}

%
\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_DynamicImpact_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_DynamicImpact_40ms}The effect of the model uncertainty terms on the engine dynamics when using the second order DSMC and how the adaptation mechanism drives the model with error to its nominal value: (a) $T_{exh}$, (b) $\dot{m}_f$, (c) $\omega_e$, and (d) $m_a$ ($T=40~ms$).} \vspace{-0.75cm}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_ParamConv_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_ParamConv_40ms}Estimation of unknown multiplicative parameters in adaptive DSMC ($T=40~ms$).} \vspace{-0.7cm}
\end{center}
\end{figure}

Fig.~\ref{fig:Engine_2DSMC_AdaptiveTracking_40ms} shows the comparison between the tracking performances of the non-adaptive and adaptive second order DSMCs. As expected, the non-adaptive DMSC fails to track the desired trajectories, which explains the importance of handling the model uncertainties in the body of the DSMC. On the other hand, once the adaptation algorithm is enabled and the convergence period of the unknown parameters is over, the adaptive DSMC tracks all the desired trajectories smoothly with the minimum error under $T=40~ms$.% ($N$ is the engine speed in terms of $RPM$). 
\vspace{-0.4cm}

\begin{figure}[h!]
\begin{center}
\includegraphics[angle=0,width= \columnwidth]{Engine_2DSMC_AdaptiveTracking_40ms.eps} \vspace{-0.75cm}
\caption{\label{fig:Engine_2DSMC_AdaptiveTracking_40ms}Comparison between adaptive and non-adaptive second order DSMCs for the engine model with uncertainties: (a) $AFR$, (b) $T_{exh}$, and (c) $N$~($T=40~ms$).} \vspace{-0.9cm}
\end{center}
\end{figure}


